3-Colouring Graphs Excluding a Fixed Minor

We show that, for every fixed graph $H$, every $n$-vertex graph $G$ that excludes $H$ as a minor is $3$-colourable with clustering $O_H(n^{4/9})$. That is, there exists a function $f$ such that for every graph $H$, every $n\ge 1$, every $n$-vertex graph $G$ that excludes $H$ as a minor has a vertex colouring with $3$ colours in which each monochromatic component has size at most $f(H)\cdot n^{4/9}$. This generalizes a recent result of Dujmovi\'c, Morin, Norin, and Wood (\textit{arXiv}:2507.03163) from planar graphs to all proper minor-closed graph classes and is the first improvement on clustered $3$-colouring of proper minor-closed graph classes since the upper bound of $O_H(\sqrt{n})$ due to Linial, Matou\v{s}ek, Sheffet, and Tardos (\textit{Comb. Prob. Comput.}, \textbf{17}(4):577--589, 2008).

==> headers/env.tex <==
\usepackage{aliascnt}
\newtheorem{theorem}{Theorem}

\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\crefname{corollary}{Corollary}{Corollaries}

\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\crefname{lemma}{Lemma}{Lemmas}

\newaliascnt{conjecture}{theorem}
\newtheorem{conjecture}[conjecture]{Conjecture}
\aliascntresetthe{conjecture}
\crefname{conjecture}{Conjecture}{Conjectures}

\newaliascnt{claim}{theorem}
\newtheorem{claim}[claim]{Claim}
\aliascntresetthe{claim}
\crefname{claim}{Claim}{Claims}

\newaliascnt{problem}{theorem}
\newtheorem{problem}[problem]{Problem}
\aliascntresetthe{problem}
\crefname{problem}{Problem}{Problems}
\crefname{pb}{Problem}{Problems}

\theoremstyle{definition}

\newaliascnt{definition}{theorem}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\crefname{definition}{Definition}{Definitions}

\newaliascnt{fact}{theorem}
\newtheorem{fact}[fact]{Fact}
\aliascntresetthe{fact}
\crefname{fact}{Fact}{Facts}

\newaliascnt{invariant}{theorem}
\newtheorem{invariant}[invariant]{Invariant}
\aliascntresetthe{invariant}
\crefname{invariant}{Invariant}{Invariants}

\newaliascnt{observation}{theorem}
\newtheorem{observation}[observation]{Observation}
\aliascntresetthe{observation}
\crefname{observation}{Observation}{Observations}

\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\crefname{proposition}{Proposition}{Propositions}

% a box
\newenvironment{bboxed}
{
  \begin{center}
    \begin{tabular}{|p{1\textwidth}|}
      \hline \\
      }
      {
      \\\\\hline
    \end{tabular}
  \end{center}
}

% notes
\newenvironment{patnote}{\par  \color{red}PM:}{\par}
\newcommand{\hussein}[1]{\textcolor{purple}{hussein: #1}}
\newcommand{\pat}[1]{\textcolor{blue}{pat: #1}}

% \newtheorem{clm}{Claim}
% \newenvironment{clmproof}{\noindent\emph{Proof of Claim:}}{\hfill{$\blacksquare$}\par}

\newcommand{\torso}[2]{#1\langle #2\rangle}


\newenvironment{clmproof}{\begin{proof}[Proof of Claim:]\renewcommand{\qedsymbol}{$\blacktriangle$}}{\end{proof}}



% Hussein: I am using this to have the same number for the same theorem.
\newtheorem{innercustomthm}{Theorem}
\newenvironment{mythm}[1]
{\renewcommand\theinnercustomthm{#1}\innercustomthm}
{\endinnercustomthm}

==> headers/packs.tex <==
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
% \usepackage{mathtools}
\usepackage[OT1]{fontenc}
\usepackage{kpfonts}
% \usepackage{svg}
% \usepackage{wasysym}
\usepackage[toc,page]{appendix}
\setcounter{secnumdepth}{4}
% \usepackage{subfig}
% \usepackage{algorithm,algpseudocode}
% \usepackage{marginnote}
\usepackage[bf,small,raggedright,compact]{titlesec}
% \usepackage[normalem]{ulem}
\usepackage[utf8]{inputenc}
% \usepackage{listings,newtxtt}
% \lstset{basicstyle=\ttfamily, keywordstyle=\bfseries}
% \usepackage{paralist}
\usepackage{enumitem}
\usepackage[dvipsnames]{xcolor}
\usepackage{hyperref}
\definecolor{linkblue}{named}{MidnightBlue}
\hypersetup{colorlinks=true, linkcolor=linkblue,  anchorcolor=linkblue,
	citecolor=linkblue, filecolor=linkblue, menucolor=linkblue,
	urlcolor=linkblue}

% \usepackage{tikz}
% \usetikzlibrary{arrows.meta}

\usepackage[english]{babel}
% \usepackage{listings,newtxtt}
% \lstset{basicstyle=\ttfamily, keywordstyle=\bfseries}

\usepackage{url}
\usepackage[nameinlink,noabbrev,capitalise]{cleveref}
\crefname{dm}{}{}
\creflabelformat{dm}{#2(DM#1)#3}
\crefname{dp}{}{}
\creflabelformat{dp}{#2(DP#1)#3}
\crefname{p}{}{}
\creflabelformat{p}{#2(#1)#3}
\crefname{bg}{}{}
\creflabelformat{bg}{#2[bg#1]#3}

% \renewenvironment{proof}{\noindent{\bfseries Proof.}}{\hfill$\blacksquare$\newline}
\renewcommand{\qedsymbol}{$\blacksquare$}
\usepackage{xpatch}
\xpatchcmd{\proof}{\itshape}{\bfseries}{}{}

\usepackage[mathlines]{lineno}
\setlength{\linenumbersep}{2em}
% \linenumbers
% \rightlinenumbers
% \linenumbers

\usepackage[longnamesfirst,numbers,sort&compress]{natbib}
\setlength{\bibsep}{0.0pt}

\titlelabel{\thetitle. \;}

\linespread{1}
\usepackage{relsize}

\usepackage[skip=8pt]{parskip}

% Source - https://tex.stackexchange.com/a/22130
% Posted by egreg
% Retrieved 2026-04-17, License - CC BY-SA 3.0

\makeatletter
\def\thm@space@setup{%
  \thm@preskip=\parskip \thm@postskip=0pt
}
\makeatother

==> headers/shortcuts.tex <==
\newcommand{\set}[1]{\{#1\}}
%\usepackage[all=normal,lists=tight]{savetrees}
%\renewcommand{\setminus}{-}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\hF}{\hat{F}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\hL}{\hat{L}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tA}{\tilde{A}}
\newcommand{\eps}{\varepsilon}
\newcommand{\opt}{\text{OPT}}
\newcommand{\vor}{\text{Vor}}
\newcommand{\dist}{\text{dist}}
\newcommand{\notetoself}[1]{\textbf{#1}}
\newcommand{\bigO}{O}
\newcommand{\cut}{\text{cut}}
\newcommand{\cact}{(g(k),f(k))\text{-cactus}}
\newcommand{\sep}{\text{sn}}
\newcommand{\del}{\text{Deletion}}
\newcommand{\bigS}{\mathcal{S}}
\newcommand{\cost}{\text{cost}}
\newcommand{\Sercost}{\text{ServiceCost}}
\newcommand{\out}{\text{out}}
\newcommand{\ins}{\text{in}}
\newcommand{\event}{\mathcal{E}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\tcalV}{\tilde{\mathcal{V}}}
\newcommand{\tO}{\tilde{O}}
\newcommand{\hnu}{\hat{\nu}}
\newcommand{\avg}{\text{avg}}
\newcommand{\vavg}{\widehat{\text{avg}}}
\newcommand{\nbcenters}{10\log n}
\newcommand{\sampled}{\eta \eps^{-6} \log^3 n}
\newcommand{\F}{\mathbb{F}}
\DeclareMathOperator{\Span}{span}
\newcommand{\aspectratio}{\Delta}

\def\eg{\textit{e.g., }}
\def\ie{\textit{i.e., }}

% Document-specific commands and math operators
\DeclareMathOperator{\len}{len}
\DeclareMathOperator{\tw}{tw}
\DeclareMathOperator{\gm}{gm}
\DeclareMathOperator{\width}{width}
\DeclareMathOperator{\pw}{pw}
\DeclareMathOperator{\bw}{bw}
\DeclareMathOperator{\td}{td}
\DeclareMathOperator{\depth}{depth}
\DeclareMathOperator{\height}{height}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\radius}{radius}
\DeclareMathOperator{\pth}{path}
\DeclareMathOperator{\mindist}{min-dist}
\DeclareMathOperator{\mindeg}{min-deg}
\DeclareMathOperator{\girth}{girth}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\boundary}{\partial}


\newcommand{\grid}{\mathlarger{\mathlarger{\boxplus}}}
